Scrutinize What We Ignore: Reining In Task Representation Shift Of Context-Based Offline Meta Reinforcement Learning

Offline meta reinforcement learning (OMRL) has emerged as a promising approach for interaction avoidance and strong generalization performance by leveraging pre-collected data and meta-learning techniques. Previous context-based approaches predominantly rely on the intuition that alternating optimization between the context encoder and the policy can lead to performance improvements, as long as the context encoder follows the principle of maximizing the mutual information between the task variable $M$ and its latent representation $Z$ ($I(Z;M)$) while the policy adopts the standard offline reinforcement learning (RL) algorithms conditioning on the learned task representation.Despite promising results, the theoretical justification of performance improvements for such intuition remains underexplored.Inspired by the return discrepancy scheme in the model-based RL field, we find that the previous optimization framework can be linked with the general RL objective of maximizing the expected return, thereby explaining performance improvements. Furthermore, after scrutinizing this optimization framework, we observe that the condition for monotonic performance improvements does not consider the variation of the task representation. When these variations are considered, the previously established condition may no longer be sufficient to ensure monotonicity, thereby impairing the optimization process.We name this issue task representation shift and theoretically prove that the monotonic performance improvements can be guaranteed with appropriate context encoder updates.Our work opens up a new avenue for OMRL, leading to a better understanding between the task representation and performance improvements.

==> Checklist/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The main claims match the theoretical and experimental results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: See Section \ref{sec:conclu_and_limit}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer:  \answerYes{}
    \item[] Justification: See Appendix \ref{sec:missing proofs}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: See Appendix \ref{sec: implemetation_details}. We also submit the source code in the supplementary.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: We submit the source code in the supplementary and will make it open-source after acceptance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: See Appendix \ref{sec: implemetation_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: All the figures we show are averaged by 4 random seeds with solid curves being mean performance and shaded areas being standard deviation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: See Section \ref{sec: reduce_training_time}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: We make sure to preserve anonymity and conform to the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNo{}
    \item[] Justification: No potential negative societal impacts are performed by this work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: See Section \ref{sec: env_settings}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: This paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> Rebuttal/rebuttal.tex <==
\section{Rebuttal}

\subsection{All Reviewer}

% openreview version
% Dear the Reviewers,
    
% We sincerely thank you for your comments! 
% We would further polish our paper.
% However, we find there exists some misunderstanding concerning our main contribution.
% Hence, we would like to restate here.

% 1. $\textbf{The clarification of our core contribution.}$

% Our paper $\textbf{does not aim to learn a better representation}$, we devote ourselves to $\textbf{further improving the training process (e.g. training stability, asymptotic performance)}$ with the task representation extraction backbone of previous works, which maximizes $I(Z;M)$, e.g. contrastive, reconstruction.
% To achieve this, we identify the task representation shift issue and rein in the task representation shift during the training process.
% Note that the classifier technique is a bonus we proposed to seek for the tuning-free property while $\textbf{our method and theoretical framework don't rely on the cross-entropy loss.}$
% $\textbf{Our method to rein the task representation shift is general}$ and can be applied to other backbones (Section 5.3).
% The convergence point of the task encoder should be the same as that of the backbone, due to the unchanged learning objective.
% Hence, $\textbf{the visualization results concerning the task representation are unnecessary, and impossible to show any difference.}$
% We kindly remind the reviewer to see Figure 1 and Figure 2, $\textbf{adding RETRO would hold lower variance over multiple seeds, more stable performance improvements, and better asymptotic performance.}$

% 2. $\textbf{The relationship between our theoretical analysis and the proposed approach.}$

% Note that $k$ in Corollary 4.11 means under the current situation, the number of samples we need to update the task encoder to achieve monotonic performance improvement.
% In general, after each update of $\textbf{the policy}$, a new $k$ needs to be computed to determine whether needs to update the task encoder.

% After each update of the policy, we would get $\epsilon_{12}^{mutual}$, and then we could compute the corresponding $k$. 
% $\textbf{If say $k=256$ and the training batch size of the task encoder is $64$. }$
% $\textbf{Now as $k=256 > 64$, the task encoder can not be updated. Then the policy would execute the next update and $\epsilon_{12}^{mutual}$ would improve. }$
% $\textbf{With new $\epsilon_{12}^{mutual}$, new $k$ would be reduced according to Corollary 4.11. If say new $k=64$, then the task encoder can be updated.}$
% In our paper, as we cannot accurately compute the value of $\epsilon_{12}^{mutual}$, we set a fixed update frequency to update the task encoder, which is indeed a manner to control the task representation shift.

% 3. $\textbf{The concerns on experiments, seeds and hyper-parameters.}$

% Though our method only runs 4 seeds per task, we just use seeds 3, 4, 5, and 6 for each task and each baseline method.
% Note that the original paper of FOCAL only uses 3 seeds to conduct the experiment.
% As for the hyper-parameter, $\textbf{our setting can cover the recommended hyper-parameters provided in their original papers.}$
% If this is not enough and the previous methods need extremely careful parameter selection, we do think our method should be the priority.
% As for Figure 1 and Figure 2, we remind the reviewer to pay more attention to the training curves.
% We don't mean the task representation shift would cause salient performance collapse.
% The task representation shift would cause the performance improvement collapse, which means $\textbf{in the training curve, the performance improvement is unstable and the variance over different seeds is large.}$
% From Figure 1 the above phenomenon is obvious, e.g. the button press, the point-robot, the dial-turn, and the ant-dir (RETRO holds the minimal variance).
% As we ensure better performance improvements, our method is more likely to achieve higher asymptotic performance (e.g. ant-dir, reach, dial-turn, button-press) with lower variance and more stable training ability.
% From Figure 2, we also do the ablation study about RETRO-FOCAL and RETRO-UNICORN to show when applying our method, the variance can be lowered, the performance improvements can be more stable and the asymptotic performance can be better. 

% 4. $\textbf{The explanation of $Z^*$, $Z_{mutual}$ and the meta-RL objective.}$

% We invite the reviewer to see line 121-123 in Section 3.2 which shows the explanation of $Z^*$.
% $\textbf{Here, we think that there exists the optimal task representation $Z^*(\cdot|x)$ that can deduce the optimal expected return}$ 
% $\textbf{which means the optimal return for any policy parameter $\theta$ is deduced by $\pi(a|s, Z^*(\cdot|x);\theta)$.}$
% Hence, based on the current policy parameter $\theta$, we only need to $\max_\theta J^*(\theta)$ to achieve the final objective.
% While for $Z_{mutual}$, it is served for maximizing mutual information $I(Z;M)$.
% $\textbf{Therfore, $Z_{mutual}$ and $Z^*$ denote two different definitions.}$
% Compared to the formalization in CSRO, $J(\pi_\theta)=\mathbb{E}\_{M\sim p(M)}[J_M(\pi_\theta)]$ where $M$ denotes the task MDP, $J_M(\pi)$ denotes $\mathbb{E}\_\tau[\sum_{t=0}^\infty \gamma^t R(s_t,a_t)]$ of the task $M$ and $\pi_\theta$ is abbreviate for $\pi_\theta(a|s,z)$, we just make it more thorough and assume existing an optimal task representation $Z^*$.
% As for the context $x$, it denotes the transition information covering $(s,a,r,s')$, which is used for encoding the task representation. 
% $\textbf{CSRO abbreviates the policy $\pi_\theta(a|s,z)$ directly as $\pi_\theta$, thereby ignoring the tasking encoding process and the expectation over $x$.}$

% ---

% In general, our work identifies a brand new issue called task representation shift, adopts a direct method to rein in the task representation shift, and finds it could bring better performance improvements, hoping to give some insights for future research concerning this issue.

Dear the Reviewers,
    
We sincerely thank you for your comments! 
We would further polish our paper.
However, we find there exists some misunderstanding concerning our main contribution.
Hence, we would like to restate here.

1. \textbf{The clarification of our core contribution.}

Our paper \textbf{does not aim to learn a better representation}, we devote ourselves to \textbf{further improving the training process (e.g. training stability, asymptotic performance)} with the task representation extraction backbone of previous works, which maximizes $I(Z;M)$, e.g. contrastive, reconstruction.
To achieve this, we identify the task representation shift issue and rein in the task representation shift during the training process.
Note that the classifier technique is a bonus we proposed to seek for the tuning-free property while \textbf{our method and theoretical framework don't rely on the cross-entropy loss.}
\textbf{Our method to rein the task representation shift is general} and can be applied to other backbones (Section 5.3).
The convergence point of the task encoder should be the same as that of the backbone, due to the unchanged learning objective.
Hence, \textbf{the visualization results concerning the task representation are unnecessary, and impossible to show any difference.}
We kindly remind the reviewer to see Figure 1 and Figure 2, \textbf{adding RETRO would hold lower variance over multiple seeds, more stable performance improvements, and better asymptotic performance.}

2. \textbf{The relationship between our theoretical analysis and the proposed approach.}

Note that $k$ in Corollary 4.11 means under the current situation, the number of samples we need to update the task encoder to achieve monotonic performance improvement.
In general, after each update of \textbf{the policy}, a new $k$ needs to be computed to determine whether needs to update the task encoder.

After each update of the policy, we would get $\epsilon_{12}^{mutual}$, and then we could compute the corresponding $k$. 
\textbf{If say $k=256$ and the training batch size of the task encoder is $64$. 
Now as $k=256 > 64$, the task encoder can not be updated. Then the policy would execute the next update and $\epsilon_{12}^{mutual}$ would improve. 
With new $\epsilon_{12}^{mutual}$, new $k$ would be reduced according to Corollary 4.11. If say new $k=64$, then the task encoder can be updated.}
In our paper, as we cannot accurately compute the value of $\epsilon_{12}^{mutual}$, we set a fixed update frequency to update the task encoder, which is indeed a manner to control the task representation shift.

3. \textbf{The concerns on experiments, seeds and hyper-parameters.}

Though our method only runs 4 seeds per task, we just use seeds 3, 4, 5, and 6 for each task and each baseline method.
Note that the original paper of FOCAL only uses 3 seeds to conduct the experiment.
As for the hyper-parameter, \textbf{our setting can cover the recommended hyper-parameters provided in their original papers.}
If this is not enough and the previous methods need extremely careful parameter selection, we do think our method should be the priority.
As for Figure 1 and Figure 2, we remind the reviewer to pay more attention to the training curves.
We don't mean the task representation shift would cause salient performance collapse.
The task representation shift would cause the performance improvement collapse, which means \textbf{in the training curve, the performance improvement is unstable and the variance over different seeds is large.}
From Figure 1 the above phenomenon is obvious, e.g. the button press, the point-robot, the dial-turn, and the ant-dir (RETRO holds the minimal variance).
As we ensure better performance improvements, our method is more likely to achieve higher asymptotic performance (e.g. ant-dir, reach, dial-turn, button-press) with lower variance and more stable training ability.
From Figure 2, we also do the ablation study about RETRO-FOCAL and RETRO-UNICORN to show when applying our method, the variance can be lowered, the performance improvements can be more stable and the asymptotic performance can be better. 

4. \textbf{The explanation of $Z^*$, $Z_{mutual}$ and the meta-RL objective.}

We invite the reviewer to see line 121-123 in Section 3.2 which shows the explanation of $Z^*$.
\textbf{Here, we think that there exists the optimal task representation $Z^*(\cdot|x)$ that can deduce the optimal expected return which means the optimal return for any policy parameter $\theta$ is deduced by $\pi(a|s, Z^*(\cdot|x);\theta)$.}
Hence, based on the current policy parameter $\theta$, we only need to $\max_\theta J^*(\theta)$ to achieve the final objective.
While for $Z_{mutual}$, it is served for maximizing mutual information $I(Z;M)$.
\textbf{Therfore, $Z_{mutual}$ and $Z^*$ denote two different definitions.}
Compared to the formalization in CSRO, $J(\pi_\theta)=\mathbb{E}_{M\sim p(M)}[J_M(\pi_\theta)]$ where $M$ denotes the task MDP, $J_M(\pi)$ denotes $\mathbb{E}_\tau[\sum_{t=0}^\infty \gamma^t R(s_t,a_t)]$ of the task $M$ and $\pi_\theta$ is abbreviate for $\pi_\theta(a|s,z)$, we just make it more thorough and assume existing an optimal task representation $Z^*$.
As for the context $x$, it denotes the transition information covering $(s,a,r,s')$, which is used for encoding the task representation. 
\textbf{CSRO abbreviates the policy $\pi_\theta(a|s,z)$ directly as $\pi_\theta$, thereby ignoring the tasking encoding process and the expectation over $x$.}

---

In general, our work identifies a brand new issue called task representation shift, adopts a direct method to rein in the task representation shift, and finds it could bring better performance improvements, hoping to give some insights for future research concerning this issue.

\subsection{Reviewer qHRG}

% openreview version
% Dear Reviewer qHRG,

% We sincerely thank you for your encouragement concerning our findings. The following are the details for your questions.

% 1. $\textbf{How to access $Z^{mutual}$?}$

% In our proof process, $Z^{mutual}$ is a theoretical convergence point concerning the objective of maximizing mutual information $I(Z;M)$.
% $\textbf{We don't aim to access it.}$
% In contrast, we use $Z^{mutual}$ to construct the upper bound of $|J^*(\theta) - J(\theta)|$ and claim that the previous works devoted to approaching $Z^{mutual}$ (reducing $|Z-Z^{mutual}|$) consistently through contrastive loss and reconstruction loss.
% Hence, these works can be covered in our return discrepancy framework.
% $\textbf{Note that the approximation error is insignificant in our paper, as our paper is to further unleash the training performance}$ based on the previous backbone.

% 2. $\textbf{A gap between Eq. (11) and Eq. (13)}$

% We thank the reviewer for proposing this problem. 
% We admit that there is a gap between Eq. (11) and Eq. (13).
% Hence, we do the following update.
% Assisted by Assumption 4.7 and Eq. (11), we can transform Eq.(13) as $|Z_2-Z_{mutual}|\le \frac{(1-\gamma)^2}{4R_{max}L_z}\epsilon^{mutual}\_{12} - \frac{1}{2}\beta, s.t. |Z_2-Z_1| \le \beta$.
% Based on the above equation, we just need to minimize $|Z_2-Z_{mutual}|$ and constrain the representation shift.
% Then, the subsequent statements in our original paper still hold.

% 3. $\textbf{Assumption 4.9 and Assumption 4.10 are hard to satisfy in practice.}$

% We admit that Assumption 4.9 and Assumption 4.10 are hard to satisfy.
% $\textbf{However, here we hope to show it is feasible in theory}$
% $ \textbf{and claim that if meeting these prerequisites, we can truly achieve monotonic performance improvements.}$
% $\textbf{And the task representation shift does indeed make a difference, which is the main contribution of our paper.}$

% 4. $\textbf{The performance dropping caused via the task representation shift is hard to observe.}$

% We invite the reviewer to see global response \#3.

% ---

% Based on the above clarifications, we hope they will address most of the reviewer's concerns.




Dear Reviewer qHRG,

We sincerely thank you for your encouragement concerning our findings. The following are the details for your questions.

1. \textbf{How to access $Z^{mutual}$?}

In our proof process, $Z^{mutual}$ is a theoretical convergence point concerning the objective of maximizing mutual information $I(Z;M)$.
\textbf{We don't aim to access it.}
In contrast, we use $Z^{mutual}$ to construct the upper bound of $|J^*(\theta) - J(\theta)|$ and claim that the previous works devoted to approaching $Z^{mutual}$ (reducing $|Z-Z^{mutual}|$) consistently through contrastive loss and reconstruction loss.
Hence, these works can be covered in our return discrepancy framework.
\textbf{Note that the approximation error is insignificant in our paper, as our paper is based on the previous backbone to further unleash the training performance.}

2. \textbf{A gap between Eq. (11) and Eq. (13)}

We thank the reviewer for proposing this problem. 
We admit that there is a gap between Eq. (11) and Eq. (13).
Hence, we do the following update.
Assisted by Assumption 4.7 and Eq. (11), we can transform Eq.(13) as $|Z_2-Z_{mutual}|\le \frac{(1-\gamma)^2}{4R_{max}L_z}\epsilon^{mutual}_{12} - \frac{1}{2}\beta, s.t. |Z_2-Z_1| \le \beta$.
Based on the above equation, we just need to minimize $|Z_2-Z_{mutual}|$ and constrain the representation shift.
Then, the subsequent statements in our original paper still hold.

3. \textbf{Assumption 4.9 and Assumption 4.10 are hard to satisfy in practice.}

We admit that Assumption 4.9 and Assumption 4.10 are hard to satisfy.
\textbf{However, here we hope to show it is feasible in theory and claim that if meeting these prerequisites, we can truly achieve monotonic performance improvements.
And the task representation shift does indeed make a difference, which is the main contribution of our paper.}

4. \textbf{The performance dropping caused via the task representation shift is hard to observe.}

We invite the reviewer to see global response \#3.

---

Based on the above clarifications, we hope they will address most of the reviewer's concerns. 


\subsection{Reviewer Mbg6}

% openreview version
% Dear Reviewer Mbg6, 

% We sincerely thank you for your thorough review. However, we find that there exist $\textbf{obvious factual errors and understanding biases}$.

% 1. $\textbf{This paper essentially relies on the supervised loss of the task label to train the encoder.}$

% We strongly disagree with the reviewer's claim and invite the reviewer to see global response \#1.


% 2. $\textbf{Meta v.s. multi-task.}$

% We strongly disagree that our paper does not belong to the offline meta-RL setting. 
% Our paper is along the path of FOCAL->CORRO->CSRO->UNICORN->RETRO (ours). 
% Noted that in your cited paper Section 6.3 $\textbf{offline outer-loop and offline inner-loop}$, they cited FOCAL as an offline meta-RL method.
% $\textbf{We don't think using task label information to assist the training of the task encoder is forbidden in the meta-RL setting.}$
% We invite the reviewer to deliberately see the statement concerning the meta-RL definition from your reference paper and note that contrastive learning-based methods are also categorized into few-shot meta-RL in Table 2.
% $\textbf{Hence, we challenge your claim concerning the setting.}$

% 3. $\textbf{The update frequency and the sample size k.}$

% We invite the reviewer to see the global response \#2.

% 4. $\textbf{The inaccuracy of theoretical analysis}$

% $\textbf{line 160-162}$: We strongly disagree that the two-phase iteration essentially optimizes the current policy.
% $\textbf{According to the definition of $J^*(\theta)$ and $J(\theta)$, two variables (e.g. policy parameter $\theta$ and task encoder $Z(\cdot|x)$) need to be optimized.}$
% $\textbf{Simply fixing the task encoder to train the policy can lead to performance improvements, but not sufficient.}$
% Hence, we need to induce the upper bound of $|J^*(\theta) - J(\theta)|$ to $\textbf{optimize the task encoder}$.
% Then, we can naturally induce the lower bound of $J^*(\theta)$ to $\textbf{optimize the policy}$.
% You can refer to [1] for a similar two-stage optimization framework in model-based RL for details.

% $\textbf{line 179-180}$: We admit that this statement may lead to confusion. 
% To better clarify our statement, we invite the reviewer to see line 178. 
% $\textbf{For policy learning, the parameter of the task encoder is fixed.}$
% $\textbf{Hence, the expectation term subtracted in line 179 is a constant concerning the policy parameter.}$
% Therefore, the equivalence should hold.

% $\textbf{line 220-221}$: Taking that the task encoder is trained from scratch. 
% Recall that $Z_{mutual}(\cdot|x)$ is the optimal task representation distribution served for maximizing $I(Z;M)$. 
% Then during the training stage, if the task representation shift $|Z_2(\cdot|x) - Z_1(\cdot|x)|$ is small, $\textbf{the term $|Z_2(\cdot|x) - Z_{mutual}(\cdot|x)|$ may become larger than the right-hand side of Eq. (11)}$ though the right-hand side becomes large also.
% We can intuitively think that this phenomenon would happen frequently during the early stage of training as $|Z_2(\cdot|x) - Z_{mutual}(\cdot|x)|$ is much larger than the $|Z_2(\cdot|x) - Z_1(\cdot|x)|$ while $\epsilon^{mutual}_{12}$ remains relatively small.

% [1] Shentao Yang et al. “A unified framework for alternating offline model training and policy
% learning”. In: Advances in Neural Information Processing Systems 35 (2022), pp. 17216–17232.

% 5. $\textbf{The weakness concerning experiments.}$

% We invite the reviewer to see global response \#1 and \#3 for clarification on experiments.

% As for the baselines IDAQ and MetaDiffuser, we do think they are irrelevant baselines as the former focuses on transition-reward distribution shift between offline datasets and online adaptation and the latter focuses on adopting diffusion as the policy to generate the action. 
% $\textbf{Our setting is fully offline (offline training and offline evaluation), which is not the setting claimed mainly in IDAQ.}$
% $\textbf{Our policy is actor-critic kind, which is not the policy adopted in MetaDiffuser.}$
% As for the baseline GENTLE, it is equivalent to UNICORN-0.
% Due to UNICORN being completely better than UNICORN-0 in this setting, it is unnecessary to compare GENTLE.

% 6. $\textbf{The explanation of $Z^*$ and the meta-learning objective.}$

% We invite the reviewer to see global response \#4.

% 7. $\textbf{The numerator of the exponential term is Equation 36 differs from the reference 37.}$

% We thank the reviewer for raising this question.
% We admit that we omit this part of derivation in the Lemma 7.2. 
% Recall that in the paper of reference 37, its result is $Pr(|P-\hat{P}|\_1 \ge\epsilon)\le (2^a-2)\exp(-m\phi(\pi\_P)\epsilon^2/4)$, where $\phi(p)=\frac{1}{1-2p}\log\frac{1-p}{p}$ and $\pi_P=\max_{A\in\mathcal{A}}\min(P(A), 1-P(A))$.
% According to the reference, $0 \le \pi_P \le 1/2, \forall P$.
% Here, we derive the function $\phi(p)$ and find that $\phi(p)$ is monotonically decreasing on $(0, 1/2)$.
% Therefore, we can get $\phi(p) \ge \phi(1/2) = 2$.
% Then, we bring this result back and can draw the conclusion that $Pr(|P-\hat{P}|_1 \ge\epsilon)\le (2^a-2)\exp(-m\epsilon^2/2)$.
% At the same time, we could get $Pr(|P-\hat{P}|_1 \le\epsilon)\ge 1 - (2^a-2)\exp(-m\epsilon^2/2)$, which is exactly the form of Eq. (36).

% As for the explanation of $vol(\mathcal{Z})$, it denotes the volume of the task representation coverage simplex.
% We admit that we made a typo in Eq. (36) and its right-hand side should be $1 - (2^{vol(\mathcal{Z})} - 2)\exp(-(N+k)\epsilon^2 / 2)$.
% Eq. (36) to Eq.(37) is for solving the $\epsilon$ from concentration inequality, which means $1-\xi = 1 - (2^{vol(\mathcal{Z})} - 2)\exp(-(N+k)\epsilon^2 / 2)$.
% Then, we could get $\epsilon$ is equal to the right-hand side of Eq. (37).
% Finally, according to the condition in Eq. (11) and Assumption 4.7, we can get Eq. (38).

% 8. $\textbf{Others.}$

% We thank the reviewer for proposing the mistakes. We would further polish our paper!

% ---

% Based on the above clarifications, we hope they will address most of the reviewer's concerns. 


Dear Reviewer Mbg6, 

We sincerely thank you for your thorough review. However, we find that there exist \textbf{obvious factual errors and understanding biases}.

1. \textbf{This paper essentially relies on the supervised loss of the task label to train the encoder.}

We strongly disagree with the reviewer's claim and invite the reviewer to see global response \#1.


2. \textbf{Meta v.s. multi-task.}

We strongly disagree that our paper does not belong to the offline meta-RL setting. 
Our paper is along the path of FOCAL->CORRO->CSRO->UNICORN->RETRO (ours). 
Noted that in your cited paper Section 6.3 \textbf{offline outer-loop and offline inner-loop}, they cited FOCAL as an offline meta-RL method.
\textbf{We don't think using task label information to assist the training of the task encoder is forbidden in the meta-RL setting.}
We invite the reviewer to deliberately see the statement concerning the meta-RL definition from your reference paper and note that contrastive learning-based methods are also categorized into few-shot meta-RL in Table 2.
\textbf{Hence, we challenge your claim concerning the setting.}

3. \textbf{The update frequency and the sample size k.}

We invite the reviewer to see the global response \#2.

4. \textbf{The inaccuracy of theoretical analysis}

\textbf{line 160-162}: We strongly disagree that the two-phase iteration essentially optimizes the current policy.
\textbf{According to the definition of $J^*(\theta)$ and $J(\theta)$, two variables (e.g. policy parameter $\theta$ and task encoder $Z(\cdot|x)$) need to be optimized.}
\textbf{Simply fixing the task encoder to train the policy can lead to performance improvements, but not sufficient.}
Hence, we need to induce the upper bound of $|J^*(\theta) - J(\theta)|$ to \textbf{optimize the task encoder}.
Then, we can naturally induce the lower bound of $J^*(\theta)$ to \textbf{optimize the policy}.
You can refer to [1] for a similar two-stage optimization framework in model-based RL for details.

\textbf{line 179-180}: We admit that this statement may lead to confusion. 
To better clarify our statement, we invite the reviewer to see line 178. 
\textbf{For policy learning, the parameter of the task encoder is fixed.}
\textbf{Hence, the expectation term subtracted in line 179 is a constant concerning the policy parameter.} 
Therefore, the equivalence should hold.

\textbf{line 220-221}: Taking that the task encoder is trained from scratch. 
Recall that $Z_{mutual}(\cdot|x)$ is the optimal task representation distribution served for maximizing $I(Z;M)$. 
Then during the training stage, if the task representation shift $|Z_2(\cdot|x) - Z_1(\cdot|x)|$ is small, \textbf{the term $|Z_2(\cdot|x) - Z_{mutual}(\cdot|x)|$ may become larger than the right-hand side of Eq. (11)} though the right-hand side becomes large also.
We can intuitively think that this phenomenon would happen frequently during the early stage of training as $|Z_2(\cdot|x) - Z_{mutual}(\cdot|x)|$ is much larger than the $|Z_2(\cdot|x) - Z_1(\cdot|x)|$ while $\epsilon^{mutual}_{12}$ remains relatively small.

[1] Shentao Yang et al. “A unified framework for alternating offline model training and policy
learning”. In: Advances in Neural Information Processing Systems 35 (2022), pp. 17216–17232.

5. \textbf{The weakness concerning experiments.}

We invite the reviewer to see global response \#1 and \#3 for clarification on experiments.

As for the baselines IDAQ and MetaDiffuser, we do think they are irrelevant baselines as the former focuses on transition-reward distribution shift between offline datasets and online adaptation and the latter focuses on adopting diffusion as the policy to generate the action. \textbf{Our setting is fully offline (offline training and offline evaluation), which is not the setting claimed mainly in IDAQ.
Our policy is actor-critic kind, which is not the policy adopted in MetaDiffuser.}
As for the baseline GENTLE, it is equivalent to UNICORN-0.
Due to UNICORN being completely better than UNICORN-0 in this setting, it is unnecessary to compare GENTLE.

6. \textbf{The explanation of $Z^*$ and the meta-learning objective.}

We invite the reviewer to see global response \#4.


7. \textbf{The numerator of the exponential term is Equation 36 differs from the reference 37.}

We thank the reviewer for raising this question.
We admit that we omit this part of derivation in the Lemma 7.2. 
Recall that in the paper of reference 37, its result is $Pr(|P-\hat{P}|_1 \ge\epsilon)\le (2^a-2)\exp(-m\phi(\pi_P)\epsilon^2/4)$, where $\phi(p)=\frac{1}{1-2p}\log\frac{1-p}{p}$ and $\pi_P=\max_{A\in\mathcal{A}}\min(P(A), 1-P(A))$.
According to the reference, $0 \le \pi_P \le 1/2, \forall P$.
Here, we derive the function $\phi(p)$ and find that $\phi(p)$ is monotonically decreasing on $(0, 1/2)$.
Therefore, we can get $\phi(p) \ge \phi(1/2) = 2$.
Then, we bring this result back and can draw the conclusion that $Pr(|P-\hat{P}|_1 \ge\epsilon)\le (2^a-2)\exp(-m\epsilon^2/2)$.
At the same time, we could get $Pr(|P-\hat{P}|_1 \le\epsilon)\ge 1 - (2^a-2)\exp(-m\epsilon^2/2)$, which is exactly the form of Eq. (36).

As for the explanation of $vol(\mathcal{Z})$, it denotes the volume of the task representation coverage simplex.
We admit that we made a typo in Eq. (36) and its right-hand side should be $1 - (2^{vol(\mathcal{Z})} - 2)\exp(-(N+k)\epsilon^2 / 2)$.
Eq. (36) to Eq.(37) is for solving the $\epsilon$ from concentration inequality, which means $1-\xi = 1 - (2^{vol(\mathcal{Z})} - 2)\exp(-(N+k)\epsilon^2 / 2)$.
Then, we could get $\epsilon$ is equal to the right-hand side of Eq. (37).
Finally, according to the condition in Eq. (11) and Assumption 4.7, we can get Eq. (38).

8. \textbf{Others.}

We thank the reviewer for proposing the mistakes. We would further polish our paper!

---

Based on the above clarifications, we hope they will address most of the reviewer's concerns. 



\subsection{Reviewer zJ2J}

% openreview version
% Dear Reviewer zJ2J, 
% We sincerely thank you for your thorough view. 
% However, we find that there exist $\textbf{obvious factual errors and understanding biases}$.

% 1. $\textbf{Previous works do not justify maximizing mutual information to improve the overall objective.}$

% We thank the reviewer for proposing this paper we ignored!
% We admit that this paper indeed considers the optimal bound and provides an in-depth analysis.
% However, this paper only gives the theoretical grounding on its own proposed algorithm, namely maximizing $I(s_{t+1},r_t;c_t|a_t)$.
% This is just a special case concerning maximizing mutual information.
% $\textbf{Our method can provide a unified theoretical grounding towards the previous works}$, covering but not limited to FOCAL, CORRO, CSRO, GENTLE, and UNICORN.
% $\textbf{These methods hold different MI maximization forms and are not considered by ContraBAR.}$

% Additionally, ContraBAR and our paper stand on different views to complete the proof process (also with different assumptions), with the former expressing the optimal policy as $\pi^*(h)$ where the $h$ denotes the history trajectory and the latter expressing the optimal policy as $\pi(a|s, Z^*(\cdot|x);\theta^*)$, where $Z^*$ denotes the optimal representation extraction from the transition.
% If we shed light on providing the theoretical grounding for transition-based methods, our work holds the first.

% 2. $\textbf{The first method to use classifier for representation learning.}$

% We strongly disagree that ContraBar adopts a classifier for representation learning by utilizing contrastive predictive coding. 
% According to the ContraBar structure, they just use MLP to achieve the dividing of positive and negative samples with InfoNCE loss.
% In contrast, $\textbf{our classifier adopts standard cross-entropy loss to train the task encoder}$, which is completely different.
% After looking through the ContraBar paper, they only adopt a binary classifier to validate the soundness of learned belief representation, \textbf{where the task encoder is not trained and the training target is only the classifier.}

% 3. $\textbf{The theoretical analysis is rather disconnected from the proposed approach.}$

% We strongly disagree with this claim and invite the reviewer to see the global response \#2.

% 4. $\textbf{Empirical evaluation is only performed on 4 seeds per task and hyper-parameters are only partially tuned}$.

% We invite the reviewer to see global response \#3.

% 5. $\textbf{Concerns on $Z^*$, $Z_{mutual}$ and decomposition.}$

% As for the distinction of $Z^*$, $Z_{mutual}$, we invite the reviewer to see global response \#4.
% As for the concern for decomposition, the logic of Section 4.1 is that the previous works have no theoretical grounding (except ContraBAR, which can only explain itself) for performance improvement, and $\textbf{we give them theoretically by introducing this decomposition.}$

% 5. $\textbf{Concerns on FOCAL and RETRO-FOCAL.}$

% We think that there may exist some understanding biases toward FOCAL.
% $\textbf{FOCAL is an end-to-end training scheme for task encoder and policy with a manner of iterative update}$.
% Hence, FOCAL does not learn a representation first and then fixed during policy training.
% Based on the above statement, RETRO-FOCAL is naturally held.

% As the reviewer alluded to the pre-training scheme, we mark pre-training can indeed avoid this problem.
% However, we empirically find that $\textbf{using the pre-training manner to train the downstream policy can not get a good performance}$ compared to normal end-to-end training.
% Hence, we focus on the end-to-end training scheme to discuss the task representation shift issue, hoping better improve the training performance.

% 6. $\textbf{Concerns on context extractor.}$

% According to our appendix Table 1 and Table 2, we maintain the task encoder of all the methods the same.

% 7. $\textbf{Concerns on visualization.}$

% We invite the reviewer to see global response \#1 for detailed clarification.

% 8. $\textbf{Concerns on title reign.}$

% We guess the reviewer would like to state the phrase $\textbf{Rein in}$ rather than $\textbf{Reign in}$.
% We are not sure whether should use $\textbf{rein in}$ in the cases of expressing the slight control.
% Here we just refer to the name of the paper <Reining Generalization in Offline Reinforcement Learning via Representation Distinction>

% 9. $\textbf{Assumption 4.7 is not imprecise.}$

% Here, we would like to show the assumption, $|Z_2-Z_1| \le \beta$.

% 10. $\textbf{Assume $Z_i$ is Gaussian.}$

% Here, we do not need to assume $Z_i$ is Gaussian, as we can model it as other distributions, e.g. beta distribution.

% 11. $\textbf{Models should be MDPs.}$

% No, here models mean the transition dynamics in the model-based RL field, which is different from the definition of MDP.

% 12. $\textbf{How is the title related to the content of the paper?}$

% Firstly, the previous works can be categorized into a return-discrepancy scheme in Section 4.1.
% They only consider consistently optimizing the task encoder to approach $Z^{mutual}$.
% Secondly, after $\textbf{scrutinizing}$ this return-discrepancy framework, we find that they $\textbf{ignore}$ the issue of task representation shift.
% By explicitly considering this, we may achieve monotonic performance improvement (Corollary 4.11), avoiding performance improvement collapse to achieve better training stability, lower variance, and higher asymptotic performance.

% 13. $\textbf{Using a cross-entropy loss the method is limited to discrete sets of tasks.}$

% We strongly disagree that our method is limited to cross-entropy loss.
% Our algorithm is general and can be applied to contrastive loss (FOCAL) and reconstruction loss (UNICORN), which is shown in Section 5.2.
% Here, the classifier loss is just an example of a backbone for the tuning-free property.

% --- 

% Based on the above clarifications, we hope they will address most of the reviewer's concerns.


Dear Reviewer zJ2J, 
We sincerely thank you for your thorough view. 
However, we find that there exist \textbf{obvious factual errors and understanding biases}.

1. \textbf{Previous works do not justify maximizing mutual information to improve the overall objective.}

We thank the reviewer for proposing this paper we ignored!
We admit that this paper indeed considers the optimal bound and provides an in-depth analysis.
However, this paper only gives the theoretical grounding on its own proposed algorithm, namely maximizing $I(s_{t+1},r_t;c_t|a_t)$.
This is just a special case concerning maximizing mutual information.
\textbf{Our method can provide a unified theoretical grounding towards the previous works}, covering but not limited to FOCAL, CORRO, CSRO, GENTLE, and UNICORN.
\textbf{These methods hold different MI maximization forms and are not considered by ContraBAR.}

Additionally, ContraBAR and our paper stand on different views to complete the proof process (also with different assumptions), with the former expressing the optimal policy as $\pi^*(h)$ where the $h$ denotes the history trajectory and the latter expressing the optimal policy as $\pi(a|s, Z^*(\cdot|x);\theta^*)$, where $Z^*$ denotes the optimal representation extraction from the transition.
If we shed light on providing the theoretical grounding for transition-based methods, our work holds the first.

2. \textbf{The first method to use classifier for representation learning.}

We strongly disagree that ContraBar adopts a classifier for representation learning by utilizing contrastive predictive coding. 
According to the ContraBar structure, they just use MLP to achieve the dividing of positive and negative samples with InfoNCE loss.
In contrast, \textbf{our classifier adopts standard cross-entropy loss to train the task encoder}, which is completely different.
After looking through the ContraBar paper, they only adopt a binary classifier to validate the soundness of learned belief representation, \textbf{where the task encoder is not trained and the training target is only the classifier.}

3. \textbf{The theoretical analysis is rather disconnected from the proposed approach.}

We strongly disagree with this claim and invite the reviewer to see the global response \#2.

4. \textbf{Empirical evaluation is only performed on 4 seeds per task and hyper-parameters are only partially tuned by approach}.

We invite the reviewer to see global response \#3.

5. \textbf{Concerns on $Z^*$, $Z_{mutual}$ and decomposition.}

As for the distinction of $Z^*$, $Z_{mutual}$, we invite the reviewer to see global response \#4.
As for the concern for decomposition, the logic of Section 4.1 is that the previous works have no theoretical grounding (except ContraBAR, which can only explain itself) for performance improvement, and \textbf{we give them theoretically by introducing this decomposition.}

6. \textbf{Concerns on FOCAL and RETRO-FOCAL.}

We think that there may exist some understanding biases toward FOCAL.
\textbf{FOCAL is an end-to-end training scheme for task encoder and policy with a manner of iterative update}.
Hence, FOCAL does not learn a representation first and then fixed during policy training.
Based on the above statement, RETRO-FOCAL is naturally held.

As the reviewer alluded to the pre-training scheme, we mark pre-training can indeed avoid this problem.
\textbf{However, we empirically find that using the pre-training manner to train the downstream policy can not get a good performance compared to normal end-to-end training.}
Hence, we focus on the end-to-end training scheme to discuss the task representation shift issue, hoping better improve the training performance.

7. \textbf{Concerns on context extractor.}

According to our appendix Table 1 and Table 2, we maintain consistency in the task encoder across all the methods.

8. \textbf{Concerns on visualization.}

We invite the reviewer to see global response \#1 for detailed clarification.

9. \textbf{Concerns on title reign.}

We guess the reviewer would like to state the phrase \textbf{Rein in} rather than \textbf{Reign in}.
We are not sure whether should use \textbf{rein in} in the cases of expressing the slight control.
Here we just refer to the name of the paper <Reining Generalization in Offline Reinforcement Learning via Representation Distinction>

10. \textbf{Assumption 4.7 is not imprecise.}

Here, we would like to show the assumption, $|Z_2-Z_1| \le \beta$.

11. \textbf{Assume $Z_i$ is Gaussian.}

Here, we do not need to assume $Z_i$ is Gaussian, as we can model it as other distributions, e.g. beta distribution.

12. \textbf{Models should be MDPs.}

No, here models mean the transition dynamics in the model-based RL field, which is different from the definition of MDP.

13. \textbf{How is the title related to the content of the paper?}

Firstly, the previous works can be categorized into a return-discrepancy scheme in Section 4.1.
They only consider consistently optimizing the task encoder to approach $Z^{mutual}$.
Secondly, after \textbf{scrutinizing} this return-discrepancy framework, we find that they \textbf{ignore} the issue of task representation shift.
By explicitly considering this, we may achieve monotonic performance improvement (Corollary 4.11), avoiding performance improvement collapse to achieve better training stability, lower variance, and higher asymptotic performance.

14. \textbf{Using a cross-entropy loss the method is limited to discrete sets of tasks.}

We strongly disagree that our method is limited to cross-entropy loss.
Our algorithm is general and can be applied to contrastive loss (FOCAL) and reconstruction loss (UNICORN), which is shown in Section 5.2.
Here, the classifier loss is just an example of a backbone for the tuning-free property.

--- 

Based on the above clarifications, we hope they will address most of the reviewer's concerns. 
